Deriving the term-structure of loan write-off risk under IFRS 9 by using survival analysis: A benchmark study

The estimation of marginal loan write-off probabilities is a non-trivial task when modelling the loss given default (LGD) risk parameter in credit risk. We explore two types of survival models in estimating the overall write-off probability over default spell time, where these probabilities form the term-structure of write-off risk in aggregate. These survival models include a discrete-time hazard (DtH) model and a conditional inference survival tree. Both models are compared to a cross-sectional logistic regression model for write-off risk. All of these (first-stage) models are then ensconced in a broader two-stage LGD-modelling approach, wherein a loss severity model is estimated in the second stage. In expanding the model suite, a novel dichotomisation step is introduced for collapsing the write-off probability into a 0/1-value, prior to LGD-calculation. A benchmark study is subsequently conducted amongst the resulting LGD-models. We find that the DtH-model outperforms other two-stage LGD-models admirably across most diagnostics. However, a single-stage LGD-model still had the best results, likely due to the peculiar `L-shaped' LGD-distribution in our data. Ultimately, we believe that our tutorial-style work can enhance LGD-modelling practices when estimating the expected credit loss under IFRS 9.

==> 3.2-Sampling.tex <==
\subsection{A diagnostic measure for testing the representativeness of resampled LGD datasets}
\label{app:resolutionRate}

% Resolution rate
As discussed by \citet{botha2025discTimeSurvTutorial}, the training and validation sets $\left\{\mathcal{D}_T, \mathcal{D}_V \right\}$ should not exhibit undue sampling bias over time. We can measure this bias using the \textit{resolution rate}, which can be calculated for either set and compared to that of the panel dataset $\mathcal{D}$.
Consider now that $\mathcal{D}$ can be partitioned into a series of non-overlapping monthly spell cohorts $\mathcal{D}(t')$ over reporting time $t'=t_1',\dots,t_l',\dots,t_n'$, e.g., Jan-2008 to Dec-2022. Let $r_\psi\left(t'_l,\mathcal{D}\right)$ denote the resolution rate at which spells resolve at any time $t'_l$ into a specified type $\psi$ within a given dataset $\mathcal{D}$. The type $\psi\in\{1,2,3\}$ refers respectively to write-off (1), cured (2), or censored (3) outcomes. Suppose that $n_{t'}$ denotes the size of $\mathcal{D}(t')$ at $t'$. Now suppose that $\mathcal{D}(t')$ contains all spells that commonly stop  at $t'$, i.e., the so-called `cohort-end'-definition from \citet{botha2025recurrentEvents}, which resolves into the resolution date. We then define the resolution rate of type $\psi$ at each $t'$ as 
\begin{equation} \label{eq:ResolRate}
    r_\psi^\mathrm{D}(t',\mathcal{D}) = \frac{1}{n_{t'}} \sum_{(i,j) \, \in \, \mathcal{D}(t')} \mathbb{I}(\mathcal{R}_{ij}^\mathrm{D} = \psi) \quad \forall \  \mathcal{D}(t') \in \mathcal{D} \ \text{and for} \ \psi \in \mathcal{R}^\mathrm{D} \, ,
\end{equation}
where $\mathbb{I}(\cdot)$ is an indicator function, and $\mathcal{R}^\mathcal{D}$ is a nominal-valued random variable with realisations $\mathcal{R}_{ij}^\mathrm{D},i=1,\dots,N_d,j=1,\dots,n_i$. This resolution rate is indeed similar to the one introduced by \citet{botha2025discTimeSurvTutorial} for performing spells.



% Resolutation rate: illustration
We can now check the sets $\left\{\mathcal{D}_T, \mathcal{D}_V \right\}$ for time-dependent sampling bias using \autoref{eq:ResolRate}. In particular, the resolution rates $r_\psi^\mathrm{D}(t',\mathcal{D})$, $r_\psi^\mathrm{D}(t',\mathcal{D}_T)$, and $r_\psi^\mathrm{D}(t',\mathcal{D}_V)$ are duly calculated and compared over $t'$ towards screening for large discrepancies. This exercise is formalised by using the MAE-based \textit{average discrepancy} (AD) measure as a diagnostic from \citet{botha2025discTimeSurvTutorial}, which is expressed between any two non-overlapping sets $\mathcal{D}_1$ and $\mathcal{D}_2$ as
\begin{equation} \label{eq:ResolRate_MAE}
     \text{AD: } \quad \bar{r}_\psi^\mathrm{D} \left(\mathcal{D}_1, \mathcal{D}_2 \right) = \frac{1}{n} \sum_{t'}{\big\vert r_\psi^\mathrm{D}(t',\mathcal{D}_1) - r_\psi^\mathrm{D}(t',\mathcal{D}_2) \big\vert} \quad \forall \ t' \ \text{and for} \ \psi \in \mathcal{R}^\mathrm{D}\, .
\end{equation}
Smaller AD-values signify greater representativeness between two subsampled sets. One can calculate the AD-measure for various combinations of our datasets, which would include $\bar{r}_\psi^\mathrm{D}(\mathcal{D},\mathcal{D}_T)$, $\bar{r}_\psi^\mathrm{D}(\mathcal{D},\mathcal{D}_V)$, and $\bar{r}_\psi^\mathrm{D}(\mathcal{D}_T,\mathcal{D}_V)$.
% Illustration
We demonstrate and compare the write-off resolution rate ($\psi=1$) in \autoref{fig:ResolRate_WOff} across different samples of data. These rates clearly track major macroeconomic phenomena such as the 2008 financial crisis and the Covid-19 pandemic, during which times the resolution rates spiked dramatically. For the 2008 crisis, there is clearly a delayed effect in the resolution rate, which is simply a function of the lengthy workout process of defaults. The last spike in the resolution rates during the 2022-2023 period is ascribed to the increases in the policy rate, as set by the central bank in response to rising inflation rates at the time. This effect caused instalments to become unaffordable for many borrowers, thereby inducing default and straining collection efforts.
% Representativeness
Nevertheless, one can observe that all rates are reasonably close to another, with an AD-value of about 0.8\% between $\mathcal{D}$ and $\mathcal{D}_T$. Based on these results, we consider the resampled sets as fairly representative of $\mathcal{D}$, which bodes well for the generalisation ability of the eventual models, beyond the training data.

\begin{figure}[ht!]
    \centering
    \includegraphics[width=0.8\linewidth, height=0.47\textheight]{ResolutionRates_Def_ts_resample_Single_Facet-9357k.png}
    \caption{Comparing the resolution rates of type $\psi=1$ (Write-off) over time across the various datasets, having used residential mortgage data. The MAE-based AD-measure from \autoref{eq:ResolRate_MAE} summarises the discrepancies over time for each dataset-pair. Inspired by \citet{botha2025discTimeSurvTutorial}.}
    \label{fig:ResolRate_WOff}
\end{figure}
